The Harder You Try, The Harder You Fail: The KeyTrap Denial-of-Service Algorithmic Complexity Attacks on DNSSEC

Availability is a major concern in the design of DNSSEC. To ensure availability, DNSSEC follows Postel's Law [RFC1123]: "Be liberal in what you accept, and conservative in what you send." Hence, nameservers should send not just one matching key for a record set, but all the relevant cryptographic material, e.g., all the keys for all the ciphers that they support and all the corresponding signatures. This ensures that validation succeeds, and hence availability, even if some of the DNSSEC keys are misconfigured, incorrect or correspond to unsupported ciphers. We show that this design of DNSSEC is flawed. Exploiting vulnerable recommendations in the DNSSEC standards, we develop a new class of DNSSEC-based algorithmic complexity attacks on DNS, we dub KeyTrap attacks. All popular DNS implementations and services are vulnerable. With just a single DNS packet, the KeyTrap attacks lead to a 2.000.000x spike in CPU instruction count in vulnerable DNS resolvers, stalling some for as long as 16 hours. This devastating effect prompted major DNS vendors to refer to KeyTrap as the worst attack on DNS ever discovered. Exploiting KeyTrap, an attacker could effectively disable Internet access in any system utilizing a DNSSEC-validating resolver. We disclosed KeyTrap to vendors and operators on November 2, 2023, confidentially reporting the vulnerabilities to a closed group of DNS experts, operators and developers from the industry. Since then we have been working with all major vendors to mitigate KeyTrap, repeatedly discovering and assisting in closing weaknesses in proposed patches. Following our disclosure, the industry-wide umbrella CVE-2023-50387 has been assigned, covering the DNSSEC protocol vulnerabilities we present in this work.

==> 041-vulnerability.tex <==
\subsection{Vulnerability Evaluation\label{sec:evaluations}}
\mydraft{We test the DoS on DNS implementations in our lab. Additionally, we investigate the preconditions on a carefully selected set of online resolvers. Following ethical imperatives, we investigate preconditions for the attack and carefully craft actual attack responses to stay within nonviscious but measurable limits. This is possible due to scalability of the attack. We use response delay as a proxy for CPU load.}

% \subsection{Evaluations in the Lab}

% see https://www.usenix.org/system/files/sec21-jeitner.pdf Table 5 for more implementations
\begin{table*}[!ht]
% \newcommand{\nousr}{$^2$}
\begin{center}
\renewcommand{\arraystretch}{0.8}
   \scriptsize
% \footnotesize
% \setlength\tabcolsep{2.5pt}
\begin{tabular}{|r|l|c|l|}
    \hline
    \ignore{\rot{Type}} & \textbf{Name}               & \textbf{Vulnerable} & \textbf{Comments}   \\
%         &                        &         & known                  & Captcha? \\
    \hline
    \multirow{12}{*}{\rot{\textbf{Server Software}}}
         % & BIND9.16.1                         & \cmark & 100\% CPU load for 5s on single PoC response \\
         % & Knot Resolver 5.3.2                       & \cmark & >45\% CPU load for 1s on PoC response\\
         % & PowerDNS Recursor 4.9.0                    & \cmark & >45\% CPU load for 1s on PoC response                       \\
         % & Unbound 1.9.4                      & \cmark &  >90\% CPU load for 5s on PoC response  \\
         & Akamai CacheServe                & \cmark  & as evaluated with Ralf on 2023-11-13 \\
         & BIND9.18.2 (latest)                & \cmark & same. "shut down hung fetch while resolving..." log message \\
         & Knot Resolver 5.7.0 (latest)               & \cmark & same as 5.3.2 \\
         & PowerDNS Recursor 4.9.1 (latest)                   & \cmark & 100\% CPU for some 5s on algorithm 16 \\
         & Unbound 1.17.0 (latest)                 & \cmark &  same. 'harden-large-queries' and 'ratelimit' not helping at all \\
         & Windows Server 2019 & \cmark & vulnerable 8, 13 PoC (15 unsupported), app. 100\% CPU, sustainable \\
         & Windows Server 2021 & \cmark & vulnerable to 13; not vulnerable to RSASHA256 PoC (?)                                 \\
         & unwind (from OpenBSD7.3)                 & \cmark & uses libunbound, PoC for 13 and 14 less effective (DNSKEY semantics) \\
    % \hline
    % \multirow{4}{*}{\rot{\textbf{Forwarders}}}
         % & pi-hole              & \tbdmark  & likely vulnerable, uses a local unbound instance \\
         & Technitium 11.4.1          &   \xmark / \cmark  & heavy CPU load under continuous attack but no DoS for client queries \\
         & dnsmasq 2.80                & \cmark &  possible rr-count limit; 'validate\_rrset()' logically vulnerable \\  % could be CVE-2023-28450 as well ("resource exhaustion on overly large UDP packets"); could also be a limitation factor; investigate reason in src/dnssec.c (int validate_rrset() and related functions); could also be an error in 'dnssec_validate_by_ds()'; EDNS0 payload size restrictions applied to TCP as well?
         & stubby 0.4.3           &    \cmark & some 30-100\% CPU core usage; substantial delay + algorithm differences \\
         & systemd-resolved 253.7          &    \cmark & eventually passes unauthenticated records to client: \servfail + Answer \\
    \hline
    \multirow{5}{*}{\rot{\textbf{ODVR}}}  % "Open DNSSEC-Validating Resolvers", slang as per https://www.dns-oarc.net/oarc/services/odvr (a shut-down service)
         & Cloudflare              & \cmark &  explicitly confirmed in Mattermost \\
         & Google              & \cmark & Implicitly confirmed by statement about working on fixes  \\
         & Neustar/Vercara  & (\cmark) & (caveat: hearsay about them using Unbound from Mattermost Channel)  \\
         & OpenDNS              & (\cmark) & ?any official confirmation?    \\
         & Quad9              & \cmark &   Confirmed by John \\
    \hline
    \multirow{6}{*}{\rot{\textbf{Tool}}}
         & drill 1.7.0 (outdated?)  & \cmark  & vulnerable only with valid DNSKEYs, fails on large RRsets, uses ldns \\
         & dig 9.16.1               &    \namark &  does not validate on its own               \\
         & kdig 2.7.8             &    \namark & does not validate on its own                \\
         & delv 9.16.1              &    \cmark & uses validator logic from BIND (PoC confirmed on delv as well)                \\
         & DNSViz 0.9.4 (latest)  &    \cmark & takes very long, consumes 100\% CPU, fails with exception                \\
         & ldns-verify-zone & \cmark & uses vulnerable ldns library (verified as manually as well) \\
         & kzonechek & \cmark & shipped with Knot DNS authoritative server \\
         & named-checkzone & \namark & does not validate signatures (named-compilezone: same) \\
         & pdnsutil & \tbdmark & (requires zone configured under running PowerDNS) \\
         
    \hline
    \multirow{6}{*}{\rot{\textbf{Library}}}
         % & coredns              &    \cmark & ?uses ldns? \\  % nice project, but not too significant
         & dnspython              &    \cmark & acc. dnssec.py:464/389 \\
         & getdns                & \tbdmark & (likely vulnerable, used by stubby)                   \\
         & go dnssec        & \namark   & validation logic limited to individual key-signature pairs \\
         & libval                & \tbdmark &                    \\
         & ldns                & \cmark & acc. dnssec\_verify.c:1142                   \\
         & libunbound              &    \tbdmark &  likely vulnerable, ?used by Unbound?        \\
    % \multirow{4}{*}{\rot{DANE}}
    %      & Exim              &    \tbdmark &                 \\
    %      & Postfix              &    \tbdmark &                 \\
    %      & Halon              &    \tbdmark &                 \\
    %      & GnuPG              &    \tbdmark &                 \\
    % \hline
    % \multirow{4}{*}{\rot{Firewalls/IDSs/Routers/Appliances}}
    %      & pfsense/opnsense              &    \tbdmark &                 \\
    %      & OpenWRT              &    \tbdmark &                 \\
    %      & FritzBox              &    \tbdmark &                 \\
    %      & Barracuda NGFW              &    \tbdmark &                 \\
    \hline
\end{tabular}
\end{center}
% \vspace{-10pt}
% \centering \footnotesize -: No response. ${}^1$: Can be retrieved using domain name/Email.
% \vspace{-8pt}
%\centering \footnotesize \nousr: Could not be determined due to unability to create a user account.
\caption{Vulnerability of Implementations. \mynote{Attack by Answer Validation only!}}
\label{tab:vulnerable:implementations}
\end{table*}

\mydraft{{\bf Preliminary PoC results.} 
Preliminary results on the first crude PoC when attacking Answer Validation (Section \ref{sec:attack-by-answer-validation}). Tested with 150 DNSKEYs and 150 RRSIGs, i.e. app. 22.5k evaluations per TCP response. We could ramp things up to about 500k validations per response (not in this first PoC to proceed faster) and esp. use more than one TCP response in the attacks. Observing algorithms 8, 13, 15. Note that not all resolvers support 15. Note that some resolvers may be not the most recent ones, but still supported. Note that the public key fields ind the DNSKEYs and the signature fields in the RRSIGs don't necessarily follow the required semantics, leading to fast failure. I.e., we can increase effectivity of the attack by a more elaborate DNSKEYs/RRSIG duplication mechanism.
All resolvers are hosted on VMs utilizing at least one Intel Xeon Gold 6142 Core @ 2.60GHz, which is pretty beefy -- launched Q3 2017 with 16 physical cores per CPU, hyper threading and a power budget of 150W.
PoC attacker NS CPU utilization is negligible (only needs to create a few TCP responses per minute with one valid, online-generated signature per response). An overview over the results is given in Table \ref{tab:vulnerable:implementations}. \\
\textbf{PowerDNS 4.6.0}: Definitely vulnerable: CPU load increases to ~45\% for about 1s on all tested algorithms\\
\textbf{Unbound 1.6.7}: Definitely vulnerable: CPU load increases to ~90\% for about 1-5s on the tested algorithms, 15 is most successful (but all have same validation pair counts)\\
\textbf{Unbound 1.17.0} (most recent version): Definitely vulnerable as well: sustained, blocking (one after another, sent-via-TCP) client queries from multiple threads are sufficient to hog up a lot of CPU resources to the point that no client queries are responded to (before generous timeout). Stopping unbound (SIGTERM?) blocks as well. 'harden-large-queries' configuration option does not make any difference (?does it not affect query responses?) and is disable by default acc. documentation (enabled by default in the docker image). ratelimit and ip-ratelimit do not make any difference, since we're using a very small number of queries per time unit only. Attack takes minutes to cool down at the resolver after stopping sending of queries. \\
\textbf{BIND 9.16.0}: Definitely vulnerable: CPU load increases to ~100\% for about 5s on 8, response for algo num 13 takes long but does not hog up CPU load(???), 15 hogs up ressources like 8\\
\textbf{Knot Resolver 5.3.2}: Definitely vulnerable: CPU load increases to ~45\% for about 1s on 8; fast response on 13(???); 15 is not supported (leading to instantaneous delivery of the records covered by our invalid RRSIGs)\\
\textbf{Windows Server 2022}: Likely vulnerable: not vulnerable for 8(!?; fast response), but takes some ~3s to respond to 13; 15 not supported; likely does syntax checks on the keys or something\\
\textbf{dnsmasq 2.80}: \sout{responses for PoC records take very long and eventually SERVFAIL, but no increased CPU usage} upstream resolver (PowerDNS) did validations (!despite CD!) and got DoS'ed; re-test with non-validating upstream resolver was clear 'invulnerable' (all-algorithm RRsets on PoC domains classified 'bogus'); classifies (valid) bloated DNSKEY set as 'bogus' as well, classifies response with valid RRSIG plus bloated invalid RRSIGs 'bogus' as well. Does not issue a DNSKEY query in the PoC (tested on 13), but apparently decides 'bogus' without it. Likely some RRset or response-size limitation mechanism. Could also be a "lucky" bug when handling overly large messages. Re-test on slimmed-down PoC (poc-sz-sig-zd-an-mis-spoc-kbf-sts-a10) yields some vulnerability: CPU load will rise to 60\% of one core, regardless of attacker counts, and client queries will be substantially delayed (about 300ms instead of 15ms until response). Confirmed that the delay is not due to processing delays at the NS (maximum service time over all responses since start is 24ms). Will apparently only validate if client is willing to accept response, since it does not validate when querying over UDP without TCP fallback (dig +notcp +ignore). \\  % DONE: check whether it maybe applies hard EDNS0 UDP payload size limitations to TCP responses -> apparently not, will accept 17,676 octets soft-PoC responses; # for i in {1000..100000}; do echo "dig @141.12.174.62 -p 5354 -t A -q session-si${i}.test-poc-sz-sig-zd-an-mis-spoc-kpg-sts-ce16.vlky.inetstudies.net."; done | parallel -j 150 bash -c
\textbf{ldns} (NLnet library for DNS debugging, used by, e.g., drill): definitely vulnerable, see calling hierarchy of dnssec\_verify.c from line 1142 on (i.e. ldns\_verify() calls ldns\_verify\_time() defined @ 1098 to validate all signatures against all keys, which iterates over the list of RRSIGs and calls ldns\_verify\_rrsig\_keylist\_time() on each individual RRSIG, which will check the RRSIG against all given keys. Note that ldns\_verify\_rrsig\_keylist\_time() will apparently use only the validation result of the last checked RRSIG, which is non-conformant with RFCs, i.e. the validation results of all non-last RRSIGs do not matter at all, but only the result of the RRSIG passed last.). Limited impact, since this is used by drill and some other debugging tools, but presumably not in a productive resolver.\\
\textbf{dnspython} definitely vulnerable (see definition of function \_validate() in dns.dnssec.py); likely limited impact: cannot find any meaningful project that makes use of this library.
\textbf{libunbound}: used by coredns OpenDNS platform resolver unwind (recursive and forwarder) and other libraries (vulnerability status undetermined) \\
\textbf{delv}: definitely vulnerable. uses same internal validation logic as BIND9. We checked Version 9.16.1-ubuntu, which was packages with BIND9.16.1 on an Ubuntu 20.04.6 LTS and is \sout{slightly outdated} not the most recent but still supported. BIND9.16 is still supported by ISC and EOL is scheduled for 2024-03 \\ %https://kb.isc.org/docs/bind-9-end-of-life-dates
\textbf{drill}: apparently not vulnerable, but needs debugging to be sure. Identifies the PoC RRsets as 'bogus' fast and without excessive resource consumption. Does the appropriate TCP fallback. Does not fail on stuffed (but valid) DNSKEY. Does not fail on stuffed (but one valid) RRSIGs. Closest implementation to 'not vulnerable', so it's a viable goal for further analysis. invocation using 'drill -V 4 -TD -k root.key POC.DOMAIN'.  says 'No keys with the keytag and algorithm from the RRSIG found' on algorithm 15 while Unbound is vulnerable on the very same zone, possible Bug or internal limit or pre-validation of proper key semantics. Re-test on full-blown PoC with timestamp-based RRSIG duplication yields mis-association log message from drill (cannot find DNSKEY with key tag conforming to RRSIG), possible bug masking the vulnerability \\
\textbf{Technitium}: not vulnerable on first glance, but limitation of q'n'd PoC applies. identifies all bogus records quite fast. does syntax checks on the cryptographic material before actually using it. e.g., will send extended error telling that RRSIG is not point on curve for algorithm 13; does not support algorithm 15. Re-test after adapted PoC yields clear vulnerability with RRSIG duplication by validity window on algorithm 8, but only limited impact: CPU load will rise to 100\% for one thread when under continious attack by $4$ clients (while the attacker NS load stays very moderate, only rises to some 10\%, likely due to our TCP implementation), will still respond to client queries for names in other zones without noticable service time increase\\
\textbf{dnsviz}: definitely vulnerable. consumes full thread at 100\%. kinda simply does its job by doing so. eventually fails with a (vague) exception, though (do bug report?). \\
\textbf{systemd-resolved}: definitely vulnerable but \emph{very} strange behavior: will take long (some seconds) to respond and consume 100\% CPU (core) resources on on RSA-based algorithms. will eventually deliver the unauthenticated records to the client along with a subset of the invalid RRSIGs in a 4k octet UDP \servfail response with AD unset. rejects TCP altogether (possible configuration error). does not consume resources on 13, 14, 15 and 16, but directly delivers the answer records (AD unset), without any accompanying RRSIGs. Supports algorithms 5, 7, 8, 10, 13, 14, and 15, but not 16. When testing for a supported algorithm (by resolving an Address record with a single, invalid-signature RRSIG), systemd-resolved will send a SERVFAIL response upstream with the address record in the Answer section and the (invalid) signature in the Additional section (which is non-conformant with [RFC4035]: RRSIGs must placed in the same section and the invalid signatures must not lead to records passed to the client). When testing for the unsupported algorithm 16, systemd-resolved will send a NOERROR response upstream, carrying only the answer RRset (located in the Answer section), but not the RRSIG covering it (missing RRSIG might be non-conformant). AD was always unset in the algorithm test responses to the client. Note that exposing systemd-resolved to the network is a relatively late feature, probably experimental. Could most likely still be attacked in pure stub mode, though. \\
\textbf{stubby}: is a privacy-focused forwarder developed as a side-product of the getdns library by NLNet and others. Definitely vulnerable, 8 and 13 apparently less so (efficient'ish processing), but 16 consumes 100\% resources. \\
\textbf{unwind}: Is the resolver of OpenBSD, the "proactively secure Unix-like operating system", which brought us OpenSSH. We tested on an up-to-date OpenBSD 7.3 ("release"; the actual Unwind version number is hard to come by...); Unwind is definitely vulnerable. Does not support 16. 15 seems very effective. Error message for 13 and 14 is 'use of key for crypto failed' (indicating our public keys can be optimized), otherwise it's 'signature crypto failed' (implying the keys were used for pubkey crypto in the first place). 13 and 14 are much less effective but still noticeably resource-intense (~1s at 45\%). Others are about 1-2s at 100\%.
}

% Stubs without validation support (adns, udns, glibc, ...) not considered here

\mydraft{
{\bf Preliminary PoC limitations.} Two limitations, both are just due to q'n'd PoC development and can be overcome/optimized.
First, DNSKEYs and RRSIGs are frequently not semantically valid, e.g. the public key field in a DNSKEY record is adjusted to have the record conform to a given key tag, but side conditions on what constitutes a semantically valid public key are hurt, so the public key might not, conform, e.g., to a valid point on the P256 curve in a DNSKEY/RRSIG of algorithm 13. This might lead to fast failure in implementations, which do according checks before doing the heavy cryptographic lifting.
Second, the number of invalid RRSIG records and DNSKEY records conforming to a single, chosen Key Tag is fixed for all algorithms and therefore limited by the least space-efficient one (RSASHA256 with 2048 bit keys). We achieve about 22.5k validations per TCP response by that, but we could go much higher by fine-tuning, e.g., 500k validations per TCP response for ECDSAP256SHA256.
}


% \subsection{Measurements on the Internet}
% % up-to-date fingerprints of cache-test would be useful here...

% \mynote{We need to discuss the details of this, esp. if the methodology is admissable. Also, note that this section only deals with the straightforward variant of the attack, not any other attack vectors.}
% \mydraft{
% We provide insights into vulnerability of popular open resolvers on the Internet (e.g., Google Public DNS, Cloudflare 1.1.1.1, OpenDNS).
% }

% \mydraft{
% These investigations are enabled by two convenient properties of our attacks.
% First, we can scale the attack up and down relatively freely: By choosing how many RRSIGs need to be validated against which count of DNSKEYs we directly control the upper bound of signature validations attempted by a vulnerable resolver under attack.  % BIND9 kills the "fetch" thread after some time, so the upper bound does not necessarily equal the lower bound
% Second, we can disarm the attack responses by selecting key tags not matching any DNSKEY in all RRSIGs except one. That one RRSIG matches a single DNSKEY. Resolvers abiding by [RFC6840], Section 5.12, ignore all others ("MUST" acc. to RFC6840, Sec. 5.12 "Ignoring Extra Signatures from Unknown Keys") and will efficiently identify the single RRSIG to be validated with its single matching DNSKEY.
% }

% \mydraft{
% The vulnerability status inference proceeds in two stages.
% In the first stage we measure side conditions of the attack, i.e. whether the resolver accepts a bloated DNSKEY set with all but one conforming to the same key tag, and whether the resolver accepts a response bloated with numerous RRSIG records with all but one conforming to the same key tag.
% To not accidentally attack the resolver we infer these properties in separate queries on separate domains and use a validation path with distinct, separate key tag, so that the resolver efficiently authenticates the records queried by our investigation script.
% }

% \mydraft{
% In the second stage, we use two types of requests for deriving information on the vulnerability status:
% Request type "(A)ttack" results in a DoS attack, which we scale down to a level of "sufficiently non-intrusive".
% Request type "(B)enign" results in the same responses from the NS, but in a disarmed version of the attack.
% }

% \mydraft{
% We proceed by sending the resolver a number of $n$ requests of type A and the same number of $n$ requests of type B, keeping the frequency of request the same notion of "low" in both cases. We closely observe the time between sending the request and receiving a response at the client. We then compare the response delays and assess whether they significantly deviate. %In result, we have collected data on two distributions of response times, which we can check for significant deviations using a statistical test or techniques borrows from ML, or just simply by visualization (if the differences are "obviously significant").
% }

% \mynote{Caveats: see comments}\\
% {\bf Methodology Drawbacks.}
% \begin{itemize}
%     \item The design of the disarmed responses assumes that the resolver ignored extra signatures (rather likely; following "MUST" from RFC6840). If it doesn't it might behave the same as under attack, which could yield a false negative.
%     \item Using response times as a proxy for CPU utilization works only under the assumption that the validations of one RRset are done on a single thread. If they are not, we risk a false negative.
%     \item If the validations for one RRset are done on a single thread, it will likely be occupied for a significant amount of time (when compared to benign responses). The open resolvers are (hopefully) closely monitored (e.g. PowerDNS has pretty comprehensive logging/statistics features). Our tests might get noticed and a) draw attention of a CERT/developer/admin team (with according operational costs), b) get investigated and (worst case) blogged about, c) be (seen as) unethical.
%     \item I'm not too comfortable with advanced statistics. But if the results are "obviously significant", the tests might not even require a high level of proficiency with statistics.
%     \item We'll likely need to tune the number of validations per armed+scaled-down attack response such that a) difference in CPU processing are more pronounced than network-induced differences and b) we still don't occupy too much CPU ressources. Afek et al. used 5 relatively strong attack requests, so we might actually do as well.
% \end{itemize}

% {\bf Methodology Advantages.}
% \begin{itemize}
%     \item allows us to estimate vulnerability before disclosure
%     \item even possibly allows us to collect the data before disclosure and do evaluations after disclosure (or after they have given/refused us entry to a testbed of product)
%     \item another "science'y" feature for the paper
% \end{itemize}



==> 050-impact_old.tex <==
% \section{Evaluation of the Attacks}\label{sec:impact}

% % Impact on DNS functionality (caching, pending records, inbound/outbound queries, DNSSEC validation, ...)

% ... (TBD)


% \subsection{Practical Requirements}
% Traditionally DNS messages were exchanged via UDP with legal payload sizes of up to $512$ octets [RFC1035].  %  RFC1035 Sec. 4.2.1 "UDP Usage"
% To overcome this limitation, the EDNS0 extensions introduced a mechanism for DNS clients to signal their maximum supported UDP payload size to the server [RFC6891].
% In theory, a DNS message on wire can now reach up to the maximum $2^{16}$ octets supported by UDP.
% Support for this signaling mechanism is a specification requirement for DNSSEC message exchange [RFC4035].
% Security-aware name servers \must{} support at least $1220$ octets and \should{} support $4000$ octets.
% Due to reliability and security issues induced by network layer fragmentation \cite{herzberg2013fragmentation, kent1995fragmentation}, most resolvers signal support for much less than the theoretic maximum in practice, rarely more than $4096$ octets. % RFC4035 demands 1220 octets and recommends 4000 octets (possibly has been updated later)
% Our measurements of UDP payload sizes advertised by resolvers are shown in Figure \ref{fig:resolver-edns-udp}
% % !! CAVEAT BIND9 EDSN0 payload size probing !!
% % NOTE ON EDNS0 and BIND9 (affecting measurements) -- EXCERPT FROM ISC Docs (https://kb.isc.org/docs/aa-01350)
% % "When querying a new server for the first time, named will send a EDNS query advertising a 512 byte UDP buffer. This is the most conservative EDNS message that can be sent.  If successful, subsequent queries will 'probe' the capabilities of the authoritative server by advertising successively larger EDNS sizes. When querying a known server using EDNS, named will choose a EDNS buffer size based on the history of EDNS timeouts at various advertised sizes and also on the largest successful EDNS response that it has already received from that server.  Note however that named cannot learn that a server (and the path between itself and the remote server) can support larger UDP packet sizes until it successfully receives a large response from that server. If any response results in a response with TC=1 being returned, then named will re-send the query using TCP - it will not take this opportunity to try with a larger advertised EDNS UDP packet size (because this might further delay getting a query response to the client)." - 
% \begin{figure}[htbp!]
%     \centering
%   %  \begin{adjustbox}{max width=0.45\textwidth}
%     %\includegraphics[width=.8\columnwidth]{img/resolver_algorithm_support_new.pdf}
%     \includegraphics[width=.8\columnwidth]{img/resolver_edns_udp.pdf}
%    % \end{adjustbox}
%     \caption{UDP payload sizes advertised by open and adnet resolvers, which also requested DNSSEC records (DO). \mynote{Preliminary figure from previous studies.}}
%     \label{fig:resolver-edns-udp}
% \end{figure}

% UDP is not the only protocol specified for transport of DNS messages.
% In fact, query transactions via TCP are a core feature of DNS, which was built into DNS from its very beginning to accomodate transfer of large messages.
% Follow-up specification has clarified that all DNS implementations \must{} support it [RFC7766].

% \epigraph{
% Recursive server (or forwarder) implementations MUST support TCP
% so that they do not prevent large responses from a TCP-capable
% server from reaching its TCP-capable clients.
% }{RFC7766, Section 5. "Transport Protocol Selection"}

% Recent studies measure support rates for DNS over TCP of between $25.0\%$ and $97.3\%$ \cite{kosek2022measuring, mao2022assessing}. \mynote{Caveats with Mao citation; Kosec citation has weird results.}
% As measured in a recent study, the vast majority of DNS queries are transmitted via UDP \cite{mao2022assessing}.
% Due to the increased transmission delays associated with TCP connection setup, DNS resolvers most frequently prefer UDP over TCP.
% However, if a DNS response does not fit the advertised UDP payload limits, DNS provides a fallback mechanism: The server sets the truncated flag (TC) in the response transmitted via UDP, indicating to the client that the response did not fit the size limitations, and that it should re-issue the same query via TCP.
% When transmitted over TCP, DNS responses are prepended a two octet length specifier, which limits the maximum message size on wire to $2^{16}$ octets.
% \mydraft{Plenty of room to fit DNSKEY and RRSIG records, which are frequently sized much less than 512 octets. % TODO give some solid numbers as examples
% Since DNS record sets need to be delivered in a single response message, the larger the supported response size the higher the number of DNSKEY and RRSIG records, which can be transmitted by an attacker to a victim resolver, making the mandatory TCP support in DNS a substantial facilitator for the attack.}  % TODO give rough calculations how many records fit what example message sizes and how that affects the number of validations

% \mydraft{
% {\bf Example calculation.}
% A $2^{16}$ octet size DNS response can fit more than $800$ DNSKEY records of algorithm ECDSAP256SHA256 (approximately $80$ octets per DNSKEY record).
% Similarly, more than $620$ RRSIG records conforming to that algorithm can fit one TCP response.
% In our attack, the DNSKEY set and the RRSIGs to be validated are transmitted in separate responses (one response filled with DNSKEYs and a single, valid and easy to validate RRSIG, one response filled with invalid RRSIGs and a single non-DNSKEY answer record).
% Therefore, a vulnerable resolver will validate more than $496\,000$ DNSKEY-RRSIG pairs for a single non-DNSKEY TCP response.
% In their $2015$ blog post\footnote{\url{https://blog.cloudflare.com/go-crypto-bridging-the-performance-gap/}}, Cloudflare tested their back-then high performance ECDSA implementaion and measured one validation would take $146\,991$ns on a single Haswell CPU core.
% Accordingly, this implementation would have taken about $73.91s$ on the tested platform to calculate through the RRSIGs in a single TCP response carrying the RRSIGs.
% Note that the attacker can send a multitude of such TCP responses for as long as the resolver is capable of processing requests.
% }
% \mynote{TCP session management might make it an inferior protocol for RRSIG transmission, e.g. in case there is no TCP connection re-use from the resolver. We might want to evaluate UDP as well.}


